code2vec: Learning Distributed Representations of Code

We present a neural model for representing snippets of code as continuous distributed vectors ("code embeddings"). The main idea is to represent a code snippet as a single fixed-length $\textit{code vector}$, which can be used to predict semantic properties of the snippet. This is performed by decomposing code to a collection of paths in its abstract syntax tree, and learning the atomic representation of each path $\textit{simultaneously}$ with learning how to aggregate a set of them. We demonstrate the effectiveness of our approach by using it to predict a method's name from the vector representation of its body. We evaluate our approach by training a model on a dataset of 14M methods. We show that code vectors trained on this dataset can predict method names from files that were completely unobserved during training. Furthermore, we show that our model learns useful method name vectors that capture semantic similarities, combinations, and analogies. Comparing previous techniques over the same data set, our approach obtains a relative improvement of over 75%, being the first to successfully predict method names based on a large, cross-project, corpus. Our trained model, visualizations and vector similarities are available as an interactive online demo at http://code2vec.org. The code, data, and trained models are available at https://github.com/tech-srl/code2vec.

==> abstract.tex <==
\begin{abstract}
%We present a novel neural network architecture for predicting method names in programs. Prediction of method names is an important task that can significantly improve code quality and code readability. The main idea of our approach is a (soft-)~attention mechanism that attends to paths in the program's abstract syntax tree. This allows our architecture to take advantage of the structured nature of code, rather than treat it as a linear token stream.
%The effectiveness of our approach is demonstrated by using it to predict methods names based on more than 14 M methods and 16 GB of training data. We show that our approach achieves F1 score of {\fscore}, increasing the F1 score obtained by previous models by relatively more than \%75. 	

%We present a model for learning continuous distributed vector representations for arbitrary-sized snippets of code.
%The main idea of our approach is a (soft-)attention mechanism that attends to \emph{paths} in the code's abstract syntax tree.
%This allows our architecture to take advantage of the structured nature of code, rather than treat it as a linear token stream. The model represents each snippet of code as a dense vector which is trained to predict a tag, caption or name. Followed by the attention mechanism, the model is interpretable and provides interesting observations about the attention that each path is given in a specific prediction.
%
%The effectiveness of our approach is demonstrated by prediction of method names, based on more than $14$M methods and $60$GB of training data. We show that our approach yields a relative improvement of over $75\%$ over previous works, and provides interesting semantic similarities and analogies between method names.

We present a neural model for representing arbitrary-sized snippets of code as continuous distributed vectors.
While some models read code as a linear token stream, our model uses the set of paths in the code's abstract syntax tree as its input, allowing it to take advantage of the structured nature of code.
These paths are then aggregated via an attention mechanism, which learns how to aggregate multiple contexts into a single fixed-length vector simultaneously with the training of the model. 
The aggregated vector can then be used to predict semantic properties of the snippet.

We demonstrate the effectiveness of our approach by using it to predict a method's name from the vector representation of its body. We evaluate our approach by training a model on a dataset of $14$M methods (encompassing $60$GB of training code), yielding a relative improvement of over $75\%$ upon the state of the art, as well as interesting semantic similarities between method names.


\end{abstract}



==> acmart-preload-hook.tex <==
\PassOptionsToPackage{dvipsnames}{xcolor}
%\PassOptionsToPackage{breaklinks=true}{hyperref}

==> intro.tex <==
\section{Introduction}\seclabel{Intro}

\ignore{
    \Distributed representations of words \cite{mikolovEfficient2013, mikolovDistributed2013}, sentences, paragraphs and documents \cite{doc2vec} played a key role in unlocking the potential of neural networks for natural language processing tasks~\cite{collobert2008, SocherEtAl2011:RNN, turian2010, glorot2011domain, turney2006similarity}. The main idea of a distributed representation is to learn low-dimensional vector representations for objects, referred to as \emph{embeddings}, such that semantically similar objects are mapped to close vectors. In neural networks learning from discrete inputs (such as in natural language processing), learning embeddings is often the first layer of the network.

\subsection{Our approach}
}

\input{soft-landing}


We present a neural network that learns \emph{code vectors} - continuous distributed vector representations for code. Our neural network architecture uses a representation of code snippets that leverages the structured nature of source code, and learns to aggregate multiple syntactic paths into a single vector.

The input to our model is a source code snippet and a corresponding tag, label, caption, or name. The tag expresses the semantic property that we wish the network to model, for example: a name that should be assigned to the snippet, a StackOverflow tag, or the name of the method, class, or project that the snippet was taken from.
Let $\mathcal{C}$ be the code snippet and $\mathcal{L}$ be the corresponding label or tag. Our underlying hypothesis is that \emph{the distribution of labels can be inferred from syntactic paths in $\mathcal{C}$}. Our model therefore attempts to learn the tag distribution, conditioned on the code:
$P\left(\mathcal{L}|\mathcal{C}\right)$.

\subsection{Applications}

\para{Predicting method names}
We demonstrate the power and expressiveness of our approach on the task of predicting method names in a program. The problem of method name prediction is closely related to the problem of code summarization. Given a method body, we use the network to predict a descriptive name. Predicting names for program elements such as variables, methods, and classes can improve code quality by making sure that elements are given descriptive names that capture their essence \cite{Lawrie:2006:WNS:1135772.1136161, takang96, liblit2006, allamanis2015, Host:2009:DMN:1615184.1615204}.

Predicting method names is a challenging task. It requires aggregating possibly hundreds of expressions and statements from the method body into a single, descriptive method name.  The best name for a method often contains words that reflect the general, high-level purpose of the method, while the body contains the low-level details. For example, a method name may be \scode{reverse()}, while the body only contains low-level instructions such as assignments to arrays (see \cref{reverse}). Without a descriptive name, one needs to follow low-level instructions to understand the purpose of the method. \Cref{Evaluation} provides additional examples.

\para{Capturing semantic similarities between names} While learning code vectors, a parallel vocabulary of tag-vectors is learned. For method names, the method name vectors provide surprising semantic similarities and analogies. For example, abusing notation, the simple vector arithmetic: $vector(\scode{compare}) + vector(\scode{toLower}) \approx  vector(\scode{compareIgnoreCase})$. These vectors also provide useful method name similarities, for example $vector(\scode{find}) \approx vector(\scode{search}) \approx vector(\scode{lookup})$.

Similar to the famous NLP example of $vector(``king'') - vector(``man'') + vector(``woman'') \approx vector(``queen'')$ \cite{mikolov2013linguistic}, the  vectors produced by our model encode analogies that are relevant to source code, and are able to complete: \emph{``\scode{receive} is to \scode{send} as \scode{download} is to ...''} with: \emph{\scode{upload}}. \Cref{qualitative} provides additional examples.

\subsection{Challenges: Representation and Attention}

The high-level challenge is how to represent code snippets in a way that captures some semantic information, is reusable across programs, and can be used to predict properties such as a label for the snippet. This leads to two conceptual challenges:
\begin{compactitem}
\item Representing a snippet in a way that enables learning across programs, and
\item Learning which parts in the representation are relevant to prediction of the desired property.
\end{compactitem}

\para{Representation}
%
Many existing approaches represent code as a token stream \cite{allamanis2014-conventions, allamanis2013, conv16, movshovitz2013natural, white2015, Hindle:2012:NS:2337223.2337322}. However, as observed previously~\cite{phog16, Pigeon}, programming languages can benefit significantly from representations that take the structured nature of the language into account. Following~\cite{Pigeon}, we therefore use paths in the program's abstract syntax tree (AST) as our representation.

%\sectionette{Decomposing code snippets to syntactic paths}
We extract paths between nodes in the snippet's AST.
%and represent each path using a \emph{path context}, a triplet $(x_{s},p,x_{f})$, where $x_{s}$ and $x_{f}$ are values of AST leaves, and $p$ is an encoding of their connecting path in the AST. 
By representing a code block using its syntactic paths, we can capture regularities that reflect common code patterns.
%\sectionette{Structural representation of code}
We then represent the snippet as a bag (multiset) of its extracted path-contexts. The challenge is then \emph{how to aggregate a bag of contexts, and which paths to focus on for making a prediction}.

\para{Attention}
%
Intuitively, the problem is the following -- we are trying to learn a correspondence between a bag of path-contexts and a label. Creating correspondence between the exact bag of path-contexts and a label as they appear in samples of the training set is going to suffer from sparsity (even similar methods will not have the \emph{exact} same bag of path-contexts). We therefore need a mechanism that can generalize and aggregate path-contexts such that bags that should yield the same label are mapped to close vectors. 

To address this challenge, which is the focus of this paper, we use a novel path-attention network architecture. Neural attention learns how much focus (``attention'') should be given to each element in a bag of path-contexts. It allows us to precisely aggregate the information captured in each individual path-context into a single vector that captures information about the entire code snippet.

Attention models have gained much popularity recently, mainly for neural machine translation (NMT) \cite{bahdanau14, luong15}, reading comprehension \cite{levy2017zeroshot, seo2016bidirectional}, vision \cite{mnih2014, ba2014}, image captioning \cite{xu2015} and speech recognition \cite{chorowski2015attention, bahdanau2016end}. While these models are sometimes very costly in terms of training time, our neural architecture is simple enough to scale and train on millions of examples.

Our attention mechanism learns how to aggregate a bag of path contexts. Importantly, learning the attention weights is done \emph{simultaneously} while learning the embeddings. That is, we simultaneously learn a good representation for individual path-contexts and a good way to aggregate them.
\ignore{
    Each of the three components in a path-context $(x_{s},p,x_{f})$ is assigned a real vector representation, or an \emph{embedding}. The three vectors of the tuple are concatenated to represent a path-context embedding. Given a set of path-context embeddings (representing the bag of path contexts), an attention mechanism learns weights on how these embeddings should be taken into a weighted average.
}
As we show in \cref{qualitative}, the weights allocated by our attention mechanism can be visualized to understand the relative importance of each path-context in a prediction.

\para{Soft and hard attention} The terms ``soft'' and ``hard'' attention were proposed for the task of image caption generation by \citet{xu2015}. In their work, \emph{soft-attention} refers to an approach where weights are placed ``softly'' over all patches in the source image, while \emph{hard-attention} refers to selection of a single patch of the image to attend to at a time. As our model uses \emph{soft}-attention, in \cref{alternative} we compare it with alternative models of \emph{hard-attention} and \emph{no-attention}, and show that \emph{soft-attention} is more efficient for modeling code.

\subsection{Existing techniques}

Distributed representations of code identifiers were first suggested by \citet{allamanis2015}, and used to predict variable, method, and class names based on token context features.
\citet{conv16} were also the first to consider the problem of predicting method names. Their technique used a convolutional neural network where locality in the model is based on textual locality in source code.

While their technique works well when training and prediction are performed within the scope of the same project, they report poor results when used across different projects (as we reproduce in \cref{quantitative}). Thus, the problem of predicting method names based on a large corpus has remained an open problem until now. To the best of our knowledge, our technique is the first to train an effective cross-project model for predicting method names.

Syntax-based contexts have been used by \citet{decisionTrees2016, phog16}. Our work differs from these in two major aspects:
\begin{compactenum}
\item These works traverse the AST only to identify a \emph{context node}, and do not use the information contained in the path itself. In contrast, our model uses the path itself as an input to the model, and can therefore generalize using this information when a known path is observed, even when the nodes in its ends have never been seen by the model before.
\item These models attempt to find a \emph{single most informative context} for each prediction. This approach resembles \emph{hard-attention}, while we suggest to use \emph{soft-attention}, that uses several contexts for prediction, with different weights for each. We compare our model with an equivalent model that uses hard-attention in \cref{alternative}.
\end{compactenum}

%% Moved here so it appears on top of page 3, anything later than that
%% is not acceptable. Ideally, I'd like it to appear on page 2.
\input{overview-figure2}

\subsection{Results}

The main contributions of this paper are:
\begin{itemize}
\item A novel path-based attention model for learning distributed representations of arbitrary-sized snippet of source code.
\item A quantitative evaluation for predicting cross-project method names, trained on more than $14$M methods of real-world data, and compared with previous work. Our experiments show that our approach achieves significantly higher results than previous works which used Long Short-Term Memory networks (LSTMs) and Convolutional Neural Networks (CNNs).
\item A qualitative evaluation that interprets the attention that the model has learnt to give to the different path-contexts when making predictions.
\item A collection of method name embeddings, which often assign semantically similar names to similar vectors, and even allows to compute analogies using simple vector arithmetic.
\item A comparison of our neural network with alternative design architectures, showing the contribution of ``soft-attention'' over ``hard-attention'' and ``no-attention''.
\item An analysis that shows the significant advantages in terms of generalization ability and space complexity of our model, compared to previous non-neural models.
\end{itemize}






==> overview-figure-textualCode.tex <==
\begin{figure*}
\centering
\begin{minipage}{7in}
\hspace{0.2in}
\begin{tabular}{ccc}
%%%%%%%%%%%%%% Subfigure 1 %%%%%%%%%%%%%%%%
\begin{subfigure}[t]{0.3\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (a){
\lstset{language=Java, basicstyle=\tiny\ttfamily,emphstyle=\underbar,escapeinside={(*}{*)}}
\begin{lstlisting}
boolean f(Object target) {
    
    for (Object elem: this.elements) {
        if (elem.equals(target)) {
            return true;
        }
        
    }
    return false;
}
\end{lstlisting}
};
\caption{}
\figlabel{overview-a}
\end{subfigure}
%\hspace{0.2in}
%%%%%%%%%%%%%% Subfigure 2 %%%%%%%%%%%%%%%%
\begin{subfigure}[t]{0.3\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (b){
\lstset{language=Java, basicstyle=\tiny\ttfamily,emphstyle=\underbar,escapeinside={(*}{*)}}
\begin{lstlisting}
Object f(int target) {
    
    for (Object elem: this.elements) {
        if (elem.hashCode().equals(target)) {
            return elem;
        }
        
    }
    return this.defaultValue;
}
\end{lstlisting}
};
\caption{}
\figlabel{overview-b}
\end{subfigure}
\hspace{0.2in}
%%%%%%%%%%%%%% Subfigure 3 %%%%%%%%%%%%%%%%
\begin{subfigure}[t]{0.3\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (c){
\lstset{language=Java, basicstyle=\tiny\ttfamily,emphstyle=\underbar,escapeinside={(*}{*)}}
\begin{lstlisting}
int f(Object target) {
    int i = 0;
    for (Object elem: this.elements) {
        if (elem.equals(target)) {
            return i;
        }
        i++;
    }
    return -1;
}
\end{lstlisting}
};
\caption{}
\figlabel{overview-a}
\end{subfigure}

\end{tabular}

%\tikz[remember picture,overlay]\draw[line width=2mm,-latex,blue] ([xshift=5mm]a.east) -- ++(10mm,0) node[below = 2mm,black, xshift=-5mm] {\small Extract paths} ;
%\tikz[remember picture,overlay]\draw[line width=2mm,-latex,blue] (b.east) -- ++(10mm,0) node[right = 2mm,black] {};
%\tikz[remember picture,overlay]\draw[line width=2mm,-latex,blue] ([xshift=-12mm, yshift=-1mm]c.west) -- ++(10mm,0) node[right = 2mm,black] {} ;
%\tikz[remember picture,overlay]\draw[line width=2mm,-latex,blue] ([xshift=-18mm]d.west) -- ++(10mm,0) node[below = 2mm,black,text width=1cm, xshift=-5mm] {\small Embedding Lookup};
%\tikz[remember picture,overlay]\draw[line width=2mm,-latex,blue] ([xshift=5mm]d.east) -- ++(10mm,0) node[below = 2mm,black, xshift=-5mm] {Concat};
%\tikz[remember picture,overlay]\draw[line width=2mm,-latex,blue] ([xshift=-12mm]e.west) -- ++(10mm,0) node[below = 2mm,black,text width=1.5cm, xshift=-5mm] {\small Attention Network};
%\tikz[remember picture,overlay]\draw[line width=2mm,-latex,blue] ([xshift=-12mm]f.west) -- ++(10mm,0) node[below = 2mm,black,text width=1.4cm, xshift=-5mm] {\small Predict \& Interpret};
\caption{An overview of method name prediction process. A simple method (a) is parsed to construct the AST from which path-contexts are extracted (b,c). The path-contexts are represented as a distributed representation (d). An attention neural network (e) aggregates the path-contexts with differential attention to predict a likely method name (\scode{contains} in this example). Interpretation of the intermediate calculations reveals the attention that each path-context was given (f).}
\end{minipage}
\end{figure*} 

==> overview-figure.tex <==
\begin{figure*}
\centering
\begin{minipage}{7in}
\hspace{0.5in}
\begin{tabular}{lcc}
%%%%%%%%%%%%%% Subfigure 1 %%%%%%%%%%%%%%%%
\begin{subfigure}[t!]{0.4\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (a){
\includegraphics[width=0.8\linewidth, trim=0 0.9cm 0 0]{overview_images/contains-initial}
};
\caption{}
\figlabel{overview-a}
\end{subfigure}
\hspace{0.3in}
%%%%%%%%%%%%%% Subfigure 2 %%%%%%%%%%%%%%%%
\begin{subfigure}[t!]{0.4\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (b){
\includegraphics[width=0.9\linewidth]{overview_images/contains-extracted}
};
\caption{}
\figlabel{overview-b}
\end{subfigure}
&
&
\\
\\
%%%%%%%%%%%%%% Subfigure 3 %%%%%%%%%%%%%%%%
\multicolumn{3}{c}{
\begin{subfigure}[b]{0.6\textwidth}
\scriptsize
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (c){
\begin{tabular}{@{}llll@{}}
$Word_{1}$ & $Path$  & $Word_{2}$  \\
\midrule
\textbf{target}     & \textbf{VarDecId$\uparrow$Parameter$\uparrow$MethodDec$\downarrow$ReturnStmt$\downarrow$Expr}  & \textbf{false}\\
\textbf{boolean}    & \textbf{PrimitiveType$\uparrow$MethodDec$\downarrow$Parameter$\downarrow$VarDecId}  & \textbf{target}\\
\textbf{boolean}    & \textbf{PrimitiveType$\uparrow$MethodDec$\downarrow$Parameter$\downarrow$ClassOrInterfaceType}  & \textbf{object}\\
\textbf{elements}   & \textbf{NameExpr$\uparrow$FieldAccessExpr$\uparrow$Foreach$\downarrow$If$\downarrow$Call$\downarrow$NameExpr}  & \textbf{equals}\\
\bottomrule
\end{tabular}
};
\caption{}
\label{Ta:overview-c}
\end{subfigure}
}
\hspace{0.3in}
%%%%%%%%%%%%%% Subfigure 4 %%%%%%%%%%%%%%%%
\begin{subfigure}[b]{0.3\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (d){
\includegraphics[width=0.4\linewidth]{overview_images/three-matrices}
};
\caption{}
\figlabel{overview-d}
\end{subfigure}
\\
\\
%%%%%%%%%%%%%% Subfigure 5 %%%%%%%%%%%%%%%%
\begin{subfigure}[b!]{0.4\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (e){
\includegraphics[width=0.9\linewidth]{overview_images/network}
};
\caption{}
\figlabel{overview-e}
\end{subfigure}
\hspace{0.4in}
%%%%%%%%%%%%%% Subfigure 6 %%%%%%%%%%%%%%%%
\begin{subfigure}[b!]{0.4\textwidth}
\tikz[remember picture]\node[inner sep=0pt,outer sep=0pt] (f){
\includegraphics[width=1\linewidth]{overview_images/contains-predicted}
};
\caption{}
\figlabel{overview-f}
\end{subfigure}

\end{tabular}

\tikz[remember picture,overlay]\draw[line width=2mm,-latex,blue] ([xshift=5mm]a.east) -- ++(10mm,0) node[below = 2mm,black, xshift=-5mm] {\small Extract paths} ;
\tikz[remember picture,overlay]\draw[line width=2mm,-latex,blue] (b.east) -- ++(10mm,0) node[right = 2mm,black] {};
\tikz[remember picture,overlay]\draw[line width=2mm,-latex,blue] ([xshift=-12mm, yshift=-1mm]c.west) -- ++(10mm,0) node[right = 2mm,black] {} ;
\tikz[remember picture,overlay]\draw[line width=2mm,-latex,blue] ([xshift=-18mm]d.west) -- ++(10mm,0) node[below = 2mm,black,text width=1cm, xshift=-5mm] {\small Embedding Lookup};
\tikz[remember picture,overlay]\draw[line width=2mm,-latex,blue] ([xshift=5mm]d.east) -- ++(10mm,0) node[below = 2mm,black, xshift=-5mm] {Concat};
\tikz[remember picture,overlay]\draw[line width=2mm,-latex,blue] ([xshift=-12mm]e.west) -- ++(10mm,0) node[below = 2mm,black,text width=1.5cm, xshift=-5mm] {\small Attention Network};
\tikz[remember picture,overlay]\draw[line width=2mm,-latex,blue] ([xshift=-12mm]f.west) -- ++(10mm,0) node[below = 2mm,black,text width=1.4cm, xshift=-5mm] {\small Predict \& Interpret};
\caption{An overview of method name prediction process. A simple method (a) is parsed to construct the AST from which path-contexts are extracted (b,c). The path-contexts are represented as a distributed representation (d). An attention neural network (e) aggregates the path-contexts with differential attention to predict a likely method name (\scode{contains} in this example). Interpretation of the intermediate calculations reveals the attention that each path-context was given (f).}
\end{minipage}
\end{figure*} 

==> packages.tex <==
%!TEX root=draft.tex
\usepackage[dvipsnames,usenames]{color}
\usepackage{fancyvrb}
\usepackage{setspace}
\usepackage{url}
\usepackage[dvipsnames]{xcolor}
\usepackage{paralist}
\usepackage[small,compact]{titlesec}
\usepackage{setspace}
\usepackage{times}
\usepackage{paralist}
\usepackage{amsmath,amssymb,amsfonts,amsthm}
\usepackage[geometry,clock]{ifsym}
\usepackage[T1]{fontenc}
\usepackage[latin9]{inputenc}
\usepackage[dvipsnames,usenames]{color}
\usepackage{listings}
\usepackage{float}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{wrapfig}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{epsfig}
% A good source for fonts:
% http://tex.stackexchange.com/questions/213835/using-many-typewriter-fonts-in-a-single-document
\usepackage{txfonts}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{rotating}
\usepackage{mathpartir}
\usepackage{array}
\usepackage{todonotes}
\usepackage[percent]{overpic}
\usepackage{ragged2e}
\usepackage{fancybox}
%\usepackage{pstricks}
\usepackage{hyperref}
\usepackage[nolist,nohyperlinks]{acronym}
\usepackage{multirow}
\usepackage{tikz}
\usepackage{xspace} % makes sure we have spaces before next word, but not before punctuation.
\usepackage{lastpage}
%\usepackage{slashbox}
\usepackage{enumitem}
%\usepackage{enumerate}

\usepackage{mathtools} 

\usepackage{booktabs}


\usepackage{framed}




==> table-analogies.tex <==
\begin{table}[]
\footnotesize
\begin{tabular}{|ll||ll|}
\hline
A : & B     & C :     & {\ul D}           \\ \hline
open :& connect     & close : &  {\ul disconnect } \\
key : &       keys          & value :  &  {\ul values }     \\
lower : &  toLowerCase & upper : &  {\ul toUpperCase} \\
down :  &  onMouseDown & up : &  {\ul onMouseUp} \\
warning :  & warningCount & error : & {\ul errorCount} \\
value :  & containsValue & key : & {\ul containsKey }\\
start :  &  activate  & end : & {\ul inactivate }\\
receive :  & download & send : &  {\ul upload }\\
\hline
\end{tabular}
\centering
\caption{Semantic analogies between method names}
\label{analogies}
\end{table}

==> table-combinations.tex <==
\begin{table}[]
\footnotesize
\begin{tabular}{|l|l||l|}
\hline
A     & $+$B     & $\approx$C             \\ \hline
get  & value & getValue   \\
get  & connection & getConnection   \\
compare  & toLower & compareIgnoreCase   \\
equals  & toLower & equalsIgnoreCase   \\
\hline
\end{tabular}
\centering
\caption{Semantic combinations of method names }
\label{additions}
\end{table}

